Learning to Learn Transferable Attack

Transfer adversarial attack is a non-trivial black-box adversarial attack that aims to craft adversarial perturbations on the surrogate model and then apply such perturbations to the victim model. However, the transferability of perturbations from existing methods is still limited, since the adversarial perturbations are easily overfitting with a single surrogate model and specific data pattern. In this paper, we propose a Learning to Learn Transferable Attack (LLTA) method, which makes the adversarial perturbations more generalized via learning from both data and model augmentation. For data augmentation, we adopt simple random resizing and padding. For model augmentation, we randomly alter the back propagation instead of the forward propagation to eliminate the effect on the model prediction. By treating the attack of both specific data and a modified model as a task, we expect the adversarial perturbations to adopt enough tasks for generalization. To this end, the meta-learning algorithm is further introduced during the iteration of perturbation generation. Empirical results on the widely-used dataset demonstrate the effectiveness of our attack method with a 12.85% higher success rate of transfer attack compared with the state-of-the-art methods. We also evaluate our method on the real-world online system, i.e., Google Cloud Vision API, to further show the practical potentials of our method.

==> table_number_gamma.tex <==
\begin{table}[t]
\centering
\begin{tabular}{l|l|l|l}
\hline
                                           &  1            & 4        & All         \\ \hline
   RN50 &  74.43          & 28.58          & 62.20          \\
  \hline
   DN121 &  75.96          & 37.88          & 66.73          \\
  \hline
\end{tabular}
\caption{The results with different number of decay factors.}
\label{tab:ablation}
\end{table}


